Evaluating Data-Driven Co-Speech Gestures of Embodied Conversational Agents through Real-Time Interaction

Embodied Conversational Agents that make use of co-speech gestures can enhance human-machine interactions in many ways. In recent years, data-driven gesture generation approaches for ECAs have attracted considerable research attention, and related methods have continuously improved. Real-time interaction is typically used when researchers evaluate ECA systems that generate rule-based gestures. However, when evaluating the performance of ECAs based on data-driven methods, participants are often required only to watch pre-recorded videos, which cannot provide adequate information about what a person perceives during the interaction. To address this limitation, we explored use of real-time interaction to assess data-driven gesturing ECAs. We provided a testbed framework, and investigated whether gestures could affect human perception of ECAs in the dimensions of human-likeness, animacy, perceived intelligence, and focused attention. Our user study required participants to interact with two ECAs - one with and one without hand gestures. We collected subjective data from the participants' self-report questionnaires and objective data from a gaze tracker. To our knowledge, the current study represents the first attempt to evaluate data-driven gesturing ECAs through real-time interaction and the first experiment using gaze-tracking to examine the effect of ECAs' gestures.

==> tables/questionsGodspeed.tex <==
\begin{table*}
\centering
\caption{Questions taken from Godspeed Questionnaire}
~\\
\label{tab:questionsGodspeed}
\begin{tabular}{p{0.3\textwidth} p{0.64\textwidth}}
\toprule
\textbf{Dimension}		  & \textbf{Item}                                                                                                                                                  \\ \toprule
Human-likeness      & How human-like does the gesture motion appear? \\
                    & 1 2 3 4 5\\
\midrule
Animacy             & Please rate your impression of the agent on these scales: \\
                    & Dead 1 2 3 4 5 Alive\\
                    & Stagnant 1 2 3 4 5 Lively\\
                    & Mechanical 1 2 3 4 5 Organic\\
                    & Artificial 1 2 3 4 5 Lifelike\\
                    & Inert 1 2 3 4 5 Interactive\\
                    & Apathetic 1 2 3 4 5 Responsive\\
\midrule
Likeability         & Please rate your impression of the agent on these scales:\\
                    & Dislike 1 2 3 4 5 Like\\
                    & Unfriendly 1 2 3 4 5 Friendly\\
                    & Unkind 1 2 3 4 5 Kind\\
                    & Unpleasant 1 2 3 4 5 Pleasant\\
                    & Awful 1 2 3 4 5 Nice\\
\midrule
Perceived Intelligence   & Please rate your impression of the agent on these scales:\\
                         & Incompetent 1 2 3 4 5 Competent\\
                         & Ignorant 1 2 3 4 5 Knowledgeable\\
                         & Irresponsible 1 2 3 4 5 Responsible\\
                         & Unintelligent 1 2 3 4 5 Intelligent\\
                         & Foolish 1 2 3 4 5 Sensible\\

\bottomrule
\end{tabular}
\end{table*}

==> tables/questionsUES.tex <==
\begin{table*}
\centering
\caption{Questions taken from User Engagement Scale}
~\\
\label{tab:questionsUES}
\begin{tabular}{p{0.3\textwidth} p{0.64\textwidth}}
\toprule
\textbf{Dimension}	   & \textbf{Item}                                                                                               \\ \toprule
Focused Attention      & I lost myself in this experience. \\
                       & Strongly Disagree 1 2 3 4 5 Strongly Agree\\ \midrule \\
                       & I was so involved in this experience that I lost track of time.\\
                       & Strongly Disagree 1 2 3 4 5 Strongly Agree\\ \midrule\\
                       & I blocked out things around me when I was interacting with the agent.\\
                       & Strongly Disagree 1 2 3 4 5 Strongly Agree\\ \midrule\\
                       & When I was interacting with the agent, I lost track of the world around me\\
                       & Strongly Disagree 1 2 3 4 5 Strongly Agree\\ \midrule\\
                       & The time I spent interacting with the agent just slipped away.\\
                       & Strongly Disagree 1 2 3 4 5 Strongly Agree\\ \midrule\\
                       & I was absorbed in this experience.\\
                       & Strongly Disagree 1 2 3 4 5 Strongly Agree\\ \midrule\\
                       & During this experience I let myself go. \\
                       & Strongly Disagree 1 2 3 4 5 Strongly Agree\\
\bottomrule
\end{tabular}
\end{table*}
